Beyond the Needle's Illusion: Decoupled Evaluation of Evidence Access and Use under Semantic Interference at 326M-Token Scale

Long-context LLM agents must access the right evidence from large environments and use it faithfully. However, the popular Needle-in-a-Haystack (NIAH) evaluation mostly measures benign span localization. The needle is near-unique, and the haystack is largely irrelevant. We introduce EverMemBench-S (EMB-S), an adversarial NIAH-style benchmark built on a 326M-token MemoryBank. While the full MemoryBank spans 326M tokens for retrieval-based (RAG) evaluation, we evaluate native long-context models only at scales that fit within each model's context window (up to 1M tokens in this work) to ensure a fair comparison. EMB-S pairs queries with collision-tested near-miss hard negatives and gold evidence sets spanning one or more documents, validated via human screening and LLM verification. We also propose a decoupled diagnostic protocol that reports evidence access (document-ID localization) separately from end-to-end QA quality under full-context prompting. This enables consistent diagnosis for both native long-context prompting and retrieval pipelines. Across a reference-corpus ladder from domain-isolated 64K contexts to a globally shared 326M-token environment, we observe a clear reality gap. Systems that saturate benign NIAH degrade sharply in evidence access under semantic interference. These results indicate that semantic discrimination, not context length alone, is the dominant bottleneck for long-context memory at scale.

==> latex/tab/human_eval.tex <==
\begin{longtable}{ccccc}
    \caption{Human evaluation scores for 100 QAR samples. MH = Multi-Hop, MC = Multiple-Choice. Completeness and Correctness are rated on a 10-point scale; Avg Score is their arithmetic mean.}
    \label{tab:human-eval-complete} \\
    \toprule
    \textbf{ID} & \textbf{Task Type} & \textbf{Completeness} & \textbf{Correctness} & \textbf{Avg Score} \\
    \midrule
    \endfirsthead
    \multicolumn{5}{c}{\textit{(Table~\ref{tab:human-eval-complete} continued from previous page)}} \\
    \toprule
    \textbf{ID} & \textbf{Task Type} & \textbf{Completeness} & \textbf{Correctness} & \textbf{Avg Score} \\
    \midrule
    \endhead
    \midrule
    \multicolumn{5}{r}{\textit{(Continued on next page)}} \\
    \endfoot
    \bottomrule
    \endlastfoot
    1 & MH & 10.0 & 8.5 & 9.25 \\
    2 & MH & 7.5 & 10.0 & 8.75 \\
    3 & MH & 7.0 & 8.5 & 7.75 \\
    4 & MH & 8.0 & 9.0 & 8.50 \\
    5 & MH & 7.0 & 9.5 & 8.25 \\
    6 & MH & 8.0 & 9.5 & 8.75 \\
    7 & MH & 6.0 & 7.5 & 6.75 \\
    8 & MH & 6.5 & 8.5 & 7.50 \\
    9 & MH & 9.5 & 9.0 & 9.25 \\
    10 & MH & 7.0 & 9.5 & 8.25 \\
    11 & MH & 9.5 & 9.0 & 9.25 \\
    12 & MH & 9.0 & 9.0 & 9.00 \\
    13 & MH & 9.5 & 7.0 & 8.25 \\
    14 & MH & 9.5 & 6.5 & 8.00 \\
    15 & MH & 9.5 & 7.0 & 8.25 \\
    16 & MH & 9.0 & 9.0 & 9.00 \\
    17 & MC & 8.5 & 10.0 & 9.25 \\
    18 & MH & 10.0 & 8.5 & 9.25 \\
    19 & MH & 10.0 & 10.0 & 10.00 \\
    20 & MH & 10.0 & 8.0 & 9.00 \\
    21 & MH & 6.0 & 8.5 & 7.25 \\
    22 & MH & 10.0 & 10.0 & 10.00 \\
    23 & MH & 7.0 & 10.0 & 8.50 \\
    24 & MH & 10.0 & 8.5 & 9.25 \\
    25 & MH & 9.0 & 5.0 & 7.00 \\
    26 & MC & 10.0 & 8.0 & 9.00 \\
    27 & MH & 9.5 & 9.5 & 9.50 \\
    28 & MH & 9.0 & 10.0 & 9.50 \\
    29 & MH & 9.5 & 10.0 & 9.75 \\
    30 & MH & 8.0 & 10.0 & 9.00 \\
    31 & MC & 6.0 & 10.0 & 8.00 \\
    32 & MC & 6.5 & 10.0 & 8.25 \\
    33 & MH & 8.0 & 10.0 & 9.00 \\
    34 & MC & 7.5 & 9.5 & 8.50 \\
    35 & MH & 9.5 & 10.0 & 9.75 \\
    36 & MH & 9.5 & 9.5 & 9.50 \\
    37 & MH & 9.0 & 10.0 & 9.50 \\
    38 & MH & 8.5 & 7.0 & 7.75 \\
    39 & MH & 9.0 & 6.0 & 7.50 \\
    40 & MH & 7.5 & 8.5 & 8.00 \\
    41 & MH & 6.5 & 10.0 & 8.25 \\
    42 & MH & 7.5 & 10.0 & 8.75 \\
    43 & MH & 8.5 & 9.0 & 8.75 \\
    44 & MH & 7.5 & 7.0 & 7.25 \\
    45 & MH & 9.5 & 7.0 & 8.25 \\
    46 & MH & 9.0 & 9.0 & 9.00 \\
    47 & MH & 9.5 & 10.0 & 9.75 \\
    48 & MH & 9.5 & 9.0 & 9.25 \\
    49 & MH & 10.0 & 10.0 & 10.00 \\
    50 & MH & 9.0 & 10.0 & 9.50 \\
    51 & MH & 10.0 & 8.5 & 9.25 \\
    52 & MH & 10.0 & 9.0 & 9.50 \\
    53 & MH & 10.0 & 9.5 & 9.75 \\
    54 & MH & 8.5 & 8.5 & 8.50 \\
    55 & MH & 7.0 & 9.5 & 8.25 \\
    56 & MH & 9.5 & 10.0 & 9.75 \\
    57 & MH & 9.0 & 8.5 & 8.75 \\
    58 & MH & 10.0 & 10.0 & 10.00 \\
    59 & MH & 8.0 & 7.0 & 7.50 \\
    60 & MH & 8.5 & 8.5 & 8.50 \\
    61 & MH & 8.5 & 9.5 & 9.00 \\
    62 & MH & 7.5 & 8.5 & 8.00 \\
    63 & MH & 9.0 & 9.5 & 9.25 \\
    64 & MH & 6.5 & 8.0 & 7.25 \\
    65 & MH & 9.5 & 9.0 & 9.25 \\
    66 & MH & 6.0 & 10.0 & 8.00 \\
    67 & MH & 7.5 & 9.5 & 8.50 \\
    68 & MH & 8.5 & 9.0 & 8.75 \\
    69 & MH & 10.0 & 10.0 & 10.00 \\
    70 & MC & 7.0 & 9.0 & 8.00 \\
    71 & MH & 10.0 & 10.0 & 10.00 \\
    72 & MH & 10.0 & 10.0 & 10.00 \\
    73 & MH & 7.0 & 10.0 & 8.50 \\
    74 & MH & 10.0 & 8.0 & 9.00 \\
    75 & MH & 10.0 & 9.0 & 9.50 \\
    76 & MH & 9.5 & 9.0 & 9.25 \\
    77 & MH & 10.0 & 8.5 & 9.25 \\
    78 & MC & 9.5 & 9.0 & 9.25 \\
    79 & MH & 8.5 & 8.5 & 8.50 \\
    80 & MH & 8.0 & 10.0 & 9.00 \\
    81 & MH & 10.0 & 8.5 & 9.25 \\
    82 & MH & 8.5 & 8.5 & 8.50 \\
    83 & MH & 10.0 & 10.0 & 10.00 \\
    84 & MH & 10.0 & 8.5 & 9.25 \\
    85 & MH & 10.0 & 9.5 & 9.75 \\
    86 & MH & 9.0 & 9.0 & 9.00 \\
    87 & MH & 10.0 & 8.5 & 9.25 \\
    88 & MH & 9.5 & 9.0 & 9.25 \\
    89 & MH & 8.5 & 9.5 & 9.00 \\
    90 & MH & 8.0 & 9.5 & 8.75 \\
    91 & MH & 10.0 & 8.5 & 9.25 \\
    92 & MH & 9.5 & 9.5 & 9.50 \\
    93 & MH & 10.0 & 8.5 & 9.25 \\
    94 & MC & 9.5 & 9.5 & 9.50 \\
    95 & MH & 9.0 & 8.5 & 8.75 \\
    96 & MH & 9.0 & 9.5 & 9.25 \\
    97 & MH & 6.0 & 10.0 & 8.00 \\
    98 & MH & 8.0 & 10.0 & 9.00 \\
    99 & MH & 10.0 & 8.5 & 9.25 \\
    100 & MH & 10.0 & 8.5 & 9.25 \\
    \end{longtable}

==> latex/tab/qa_case_study.tex <==
\begin{figure*}[!t]
    \centering
    \begin{tcolorbox}[
        width=\textwidth,
        colback=white,
        colframe=black,
        boxrule=0.6pt,
        arc=1mm,
        left=2mm,right=2mm,top=1mm,bottom=1mm,
        title=\textbf{QA Case Study (64K/Finance, Top-10) --- Transfer Policy Query},
        fonttitle=\normalsize\bfseries
    ]
    {\scriptsize
    % colored correctness marks (local to this QA case figure)
    \newcommand{\cmark}{\textcolor{green!55!black}{\ding{51}}}
    \newcommand{\xmark}{\textcolor{red!70!black}{\ding{55}}}
    \noindent\textbf{Query:} ``If a user wants to transfer \$60,000 via China Bank's online banking on a weekday at 4:45 PM, what should they consider to ensure the transaction is processed efficiently?'' \\
    \noindent\textbf{Reference answer (key points):} The amount exceeds the real-time transfer limit; use ordinary transfer and ensure the transaction is submitted within the weekday acceptance window (9:00--17:00). If submitted near the cutoff, processing may be delayed; funds typically arrive within 24 hours.

    \vspace{2pt}
    \begin{tabular}{p{0.49\textwidth}p{0.49\textwidth}}
    \toprule
    \textbf{Qwen3-4B-Instruct-2507 (lower score)}~\xmark & \textbf{Qwen3-235B-A22B-Instruct-2507 (higher score)}~\cmark \\
    \midrule
    \textbf{Generated answer (excerpt):} \newline
    Identifies ``real-time'' vs ``ordinary'' transfer, notes 50,000 RMB limit, but the final guidance is incomplete and does not clearly conclude the acceptance-time requirement for the larger amount at 4:45 PM. \newline\newline
    \textbf{Judge score:} \textbf{1.0/5}. \newline
    &
    \textbf{Generated answer (excerpt):} \newline
    Correctly distinguishes transfer modes, states that amounts \(>50{,}000\) RMB require ``ordinary transfer,'' and highlights the weekday acceptance window (9:00--17:00). Notes that submitting at 4:45 PM is close to the cutoff and may affect processing time; ordinary transfers typically arrive within 24 hours. \newline\newline
    \textbf{Judge score:} \textbf{5.0/5}. \newline
    \\
    \bottomrule
    \end{tabular}
    }
    \end{tcolorbox}
    \caption{\textbf{QA case study:} all QA-case content is shown in a single boxed figure for compact, side-by-side comparison.}
    \label{fig:app-qa-case-transfer}
\end{figure*}

==> latex/tab/re_case_study.tex <==
\begin{figure*}[t]
    \centering
    \begin{tcolorbox}[
        width=\textwidth,
        colback=white,
        colframe=black,
        boxrule=0.6pt,
        arc=1mm,
        left=2mm,right=2mm,top=1mm,bottom=1mm,
        title=\textbf{Retrieval Case Study (1M) --- Query ID 17},
        fonttitle=\normalsize\bfseries
    ]
    {\scriptsize
    \newcommand{\qterm}[1]{\underline{\textbf{#1}}}
    % colored correctness marks (local to this retrieval case figure)
    \newcommand{\cmark}{\textcolor{green!55!black}{\ding{51}}}
    \newcommand{\xmark}{\textcolor{red!70!black}{\ding{55}}}
    \noindent\textbf{Query:} ``What were the key financial figures related to \qterm{customer} and \qterm{broker} \qterm{receivables} and \qterm{payables} as of \qterm{December 31, 2016}, and how do these compare to the \qterm{vesting} of \qterm{equity} \qterm{awards} in \qterm{2019} and the company's \qterm{share} \qterm{repurchase} activities?'' \\
    \noindent\textbf{R@10:} Linq-Embed-Mistral (left, weaker) = 0.33;\ \ Qwen3-Embedding-0.6B (right, stronger) = 1.00. \\
    \noindent\textbf{Marked terms:} Underlined terms are query-overlap tokens and close variants (e.g., \qterm{receivable(s)}, \qterm{payable(s)}, \qterm{broker}, \qterm{customer}, \qterm{vesting}, \qterm{equity}, \qterm{award(s)}, \qterm{share}, \qterm{repurchase}, and date tokens like \qterm{2016}/\qterm{2019}). \cmark/\xmark indicate whether the retrieved document is in the gold evidence set.

    \vspace{2pt}
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.08}
    \begin{tabular}{p{0.05\textwidth}p{0.46\textwidth}p{0.46\textwidth}}
    \toprule
    \textbf{Rank} &
    \textbf{\shortstack{Linq-Embed-Mistral (weaker)\\(index + excerpt)}} &
    \textbf{\shortstack{Qwen3-Embedding-0.6B (stronger)\\(index + excerpt)}} \\
    \midrule
    \#1  & \textbf{257} (\xmark) ``in millions of dollars'' table, \qterm{December} 31, \qterm{2016} (with 2017 comparison); \qterm{receivables} excerpt. & \textbf{933} (\cmark) ``in millions of dollars'' table: \qterm{December} 31, \qterm{2016}; \qterm{receivables} from \qterm{customers}/\qterm{brokers} and \qterm{payables}. \\
    \#2  & \textbf{933} (\cmark) ``in millions of dollars'' table: \qterm{December} 31, \qterm{2016}; \qterm{receivables} from \qterm{customers}/\qterm{brokers} and \qterm{payables}. & \textbf{257} (\xmark) ``in millions of dollars'' table, \qterm{December} 31, \qterm{2016} (with 2017 comparison); \qterm{receivables} excerpt. \\
    \#3  & \textbf{466} (\xmark) Operating activities snippet. & \textbf{386} (\cmark) \qterm{Vesting} of \qterm{Equity} \qterm{Awards} During \qterm{2019}; ``Stock vested during \qterm{2019}'' table. \\
    \#4  & \textbf{226} (\xmark) 2018 grant of restricted stock; \qterm{shares} / \qterm{awards} mention. & \textbf{1028} (\xmark) Brokerage \qterm{receivables} and brokerage \qterm{payables} discussion. \\
    \#5  & \textbf{1087} (\xmark) Brokerage \qterm{receivables} and brokerage \qterm{payables} discussion. & \textbf{1185} (\xmark) Liquidity resources table excerpt. \\
    \#6  & \textbf{175} (\xmark) Forfeiture estimate revision note. & \textbf{563} (\cmark) Issuer purchases of \qterm{equity} securities; \qterm{share} \qterm{repurchase} program authorization excerpt. \\
    \#7  & \textbf{1185} (\xmark) Liquidity resources table excerpt. & \textbf{1087} (\xmark) Brokerage \qterm{receivables} and brokerage \qterm{payables} discussion. \\
    \#8  & \textbf{1028} (\xmark) Brokerage \qterm{receivables} and brokerage \qterm{payables} excerpt. & \textbf{466} (\xmark) Operating activities snippet. \\
    \#9  & \textbf{808} (\xmark) Net cash used in investing activities (2018) excerpt. & \textbf{223} (\xmark) Restricted stock \qterm{awards} / \qterm{shares} table excerpt. \\
    \#10 & \textbf{557} (\xmark) Market risk / position sizing snippet. & \textbf{848} (\xmark) ``year ended'' (2019) table excerpt. \\
    \bottomrule
    \end{tabular}
    }
    \end{tcolorbox}
    \caption{\textbf{Retrieval case study (Query ID 17):} all retrieval-case content is shown in a single boxed figure for compact, side-by-side comparison.}
    \label{fig:app-retrieval-case-17}
\end{figure*}
